Compositional Generalization for Natural Language Interfaces to Web APIs

This paper presents Okapi, a new dataset for Natural Language to executable web Application Programming Interfaces (NL2API). This dataset is in English and contains 22,508 questions and 9,019 unique API calls, covering three domains. We define new compositional generalization tasks for NL2API which explore the models' ability to extrapolate from simple API calls in the training set to new and more complex API calls in the inference phase. Also, the models are required to generate API calls that execute correctly as opposed to the existing approaches which evaluate queries with placeholder values. Our dataset is different than most of the existing compositional semantic parsing datasets because it is a non-synthetic dataset studying the compositional generalization in a low-resource setting. Okapi is a step towards creating realistic datasets and benchmarks for studying compositional generalization alongside the existing datasets and tasks. We report the generalization capabilities of sequence-to-sequence baseline models trained on a variety of the SCAN and Okapi datasets tasks. The best model achieves 15\% exact match accuracy when generalizing from simple API calls to more complex API calls. This highlights some challenges for future research. Okapi dataset and tasks are publicly available at https://aka.ms/nl2api/data.

==> figures/related_work.tex <==
NL2APIs leverage semantic parsing techniques which map natural language utterances to executable formal languages such as logical forms \citep{price-1990-evaluation, Zelle1996}, SQL~\citep{Yu&al.18c, zhongSeq2SQL2017}, SPARQL~\citep{Keysers2020MeasuringCG, berant-etal-2013-semantic}, web API~\citep{Su2017,Su2018}, and dataflow programs~\citep{SMDataflow2020} for building interfaces to knowledge bases, accessing resources, question answering and instructions following in smart agents, code generation, and many other applications. In the following section, we focus on the existing datasets and methods that study compositional generalization in semantic parsing tasks.

\textbf{Datasets}\quad Several synthetic datasets and tasks have been created for investigating compositional generalization in semantic parsing including SCAN~\citep{Lake2018GeneralizationWS} which has become the primary benchmark in this field. SCAN is a corpus of natural language commands and action sequence pairs, for example, "turn left and jump" maps to "{\small\texttt{I-TURN-LEFT I-JUMP}}". There are several methods of splitting SCAN dataset to evaluate compositional generalization in different aspects. In this work, we focus on the performance of models on SCAN in the Length~\citep{Lake2018GeneralizationWS} and Maximum Compound Divergence (MCD)~\citep{Keysers2020MeasuringCG} splits. The Length split separates the training and test sets such that all the examples in test set have longer action sequence. MCD was proposed by ~\citealp{Keysers2020MeasuringCG} along with CFQ, a synthetic semantic parsing dataset. This split is based on the distribution of individual rules (atoms) and their combinations (compounds) in examples. MCD splits the dataset to train and test sets such that the divergence between the distribution of compounds in train and test sets is maximized while the atoms distribution divergence remains small.  
Moreover, another synthetic dataset called COGS~\citep{kim2020cogs} has been developed that maps sentences to logical forms and evaluates the structural and lexical generalizations. 
\citealp{Shaw2020CompositionalGA} leveraged the GeoQuery dataset~\cite{Zelle1996} to evaluate the compositional generalization on a non-synthetic dataset. GeoQuery contains questions about US geography and their representation in Functional Query Language and was split according to Length and MCD methods. %Moreover, GeoQuery and several other text-to-SQL databases were used to evaluate compositionality with respect to template or program split by ~\citealp{Herzig2020SpanbasedSP, Oren2020ImprovingCG}. Spider \cite{Yu&al.18c} is a non-synthetic dataset created with the goal of generalization to unseen databases in text-to-SQL task. Spider was used to study compositional generalization MCD split by considering all the tokens in the SQL query as atoms \cite{Shaw2020CompositionalGA}. However, we are interested in semantic parsing systems ability in generalizing from simple queries to queries which can be deduced from two or more simple queries. Splitting text-to-SQL datasets to study such a capability is not trivial. Due to the flat representation of web-API languages, the clauses in API queries are easily discernible. Therefore, the compositional challenge is to generalize to unseen combinations and ordering of these clauses. 

The task of building an end-to-end framework for transferring natural language to a given web API was introduced by \citealp{Su2017}. They created a non-synthetic dataset for email and calendar domains via crowdsourcing and evaluated sequence-to-sequence and language models against their dataset. However, their dataset is not publicly available and includes fewer domains and is smaller in size compare to Okapi. Also, it lacks diversity in questions and parameter values, and therefore is not a good representative of realistic API calls.   
We created Okapi with three criteria in mind: 1- being realistic and a good representative of actual applications, 2- having diversity in both API calls and natural language questions, and 3- high quality with respect to annotations. 

\textbf{Methods}\quad Several approaches have been developed to solve the compositional generalization tasks in the datasets mentioned in the previous section. Perfect accuracy has been achieved for SCAN splits by several specialized architecture models~\citep{Shaw2020CompositionalGA, nye2020, liu2020compositional,chen2020compositional} which learn and incorporate grammar or structure to tackle compositional generalization challenges. \citealp{Herzig2020SpanbasedSP} and \citealp{Shaw2020CompositionalGA} both evaluated their models on a subset of GeoQuery dataset splits and achieved strong performance. However the span-based semantic parsing model \citep{Herzig2020SpanbasedSP} requires manual task specific pre-processing. Moreover, \citealp{Oren2020ImprovingCG}, studied the compositional generalization on several non-synthetic text-to-SQL datasets, which proved to be challenging. Note that these models are evaluated on examples which use placeholders in place of their entities. Moreover, at this time none of these systems have publicly available code to be tested on NL2API dataset. 


Finally, \citealp{Furrer2020CompositionalGI} investigated the ability of pre-trained transformer language models in compositional generalization and found them helpful while not enough to solve it. In addition, they evaluated several specialized architectures and discovered those models do not transfer well to other datasets.



